End-to-end workflow for machine learning-based qubit readout with QICK and hls4ml

We present an end-to-end workflow for superconducting qubit readout that embeds co-designed Neural Networks (NNs) into the Quantum Instrumentation Control Kit (QICK). Capitalizing on the custom firmware and software of the QICK platform, which is built on Xilinx RFSoC FPGAs, we aim to leverage machine learning (ML) to address critical challenges in qubit readout accuracy and scalability. The workflow utilizes the hls4ml package and employs quantization-aware training to translate ML models into hardware-efficient FPGA implementations via user-friendly Python APIs. We experimentally demonstrate the design, optimization, and integration of an ML algorithm for single transmon qubit readout, achieving 96% single-shot fidelity with a latency of 32ns and less than 16% FPGA look-up table resource utilization. Our results offer the community an accessible workflow to advance ML-driven readout and adaptive control in quantum information processing applications.

==> unused/codesign-v0.tex <==
% While the full readout window is 770 ADC clock cycles, we first explore the performance of ML-based state discrimination if only a part of the data is utilized.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.3\linewidth]{fig/2_layer_NN_800_netron.png}
    \caption{NN model architecture. This here could also illustrate the structure of the training data.}
    \label{fig:modelarch}
\end{figure}

\subsection{Optimization methods}

The primary objective of the neural network model is to facilitate efficient and accurate qubit readout within the firmware design pipeline.
Recently, various neural network architectures have found direct applications with transmon qubit systems.
Recurrent neural networks (RNNs), designed for sequential data, have been utilized to infer individual quantum trajectories of a superconducting qubit's evolution~\cite{PhysRevX.10.011006, PhysRevX.12.031017}.
Autoencoders are used for superconducting qubits by pretraining on qubit readout signals to extract relevant features, which are then used for enhanced classification performance in a supervised manner \cite{PhysRevApplied.20.014045}.
For direct qubit state classification, convolutional neural networks (CNNs) and feedforward neural networks (FNNs) have been proposed due to their simplicity and ability to mitigate cross-talk effects in multi-qubit configurations \cite{PhysRevApplied.17.014024}, \cite{10.1063/5.0065011}.

In line with previous comparisons between NN models~\cite{PhysRevApplied.17.014024, 10.1063/5.0065011}, we found that different types of neural network architectures perform similarly for the qubit classification problem, with feed-forward architectures having a slight edge in classification accuracy.
Beyond accuracy, the choice of NN architecture is highly constrained by the system requirements, available FPGA resources, and strict latency constraints.
Co-design of the algorithm is a Pareto optimization between algorithm fidelity and NN resources and latency.
Dense MLPs, due to their straightforward design, often require fewer computational resources than more complex architectures like RNNs, CNNs, or autoencoders. 
% \textcolor{red}{@Omer is it true that we explored other architectures and found MLP does just as well?} \textcolor{blue}{ Indeed we have, but there are also other work from literature such as the multiqubit work from MIT making the same comparison}.  
Considering these factors, we selected a feed-forward neural network for binary classification to distinguish between the ground and excited states of qubits. 
The model's simplicity ensures effective integration into the QICK system without overwhelming computational resources, particularly within a cryogenic environment under strict thermal budgets. 
\fixme{Don't mention thermal load here, maybe put in outlook} The model comprises of Dense and Batch normalization layers. 

% \begin{enumerate}
%     \item \textbf{Linear Transformation:} This initial layer has an input size corresponding to the sampling rate (sr) and an output size of sr/4. It linearly transforms the input data using learned weights and biases. The transformation is expressed as \( y = Wx + b \), where \( W \) is the weight matrix, \( x \) is the input, and \( b \) is the bias vector. This step reduces the dimensionality of the data while preserving essential features.
    
%     \item \textbf{ReLU Activation:} The Rectified Linear Unit (ReLU) function is applied to the output of the linear transformation. It introduces non-linearity into the model by mapping \( f(x) = \max(0, x) \), enabling the network to learn and model complex patterns within the data.
    
%     \item \textbf{Batch Normalization:} A Batch Normalization layer stabilizes the activations of the neural network. This layer normalizes the activations of the previous layer to have a mean of zero and a standard deviation of one, accelerating training and improving overall performance.
    
%     \item \textbf{Linear Transformation:} A second linear layer follows, with an input size of sr/4 and an output size of 2. This layer further transforms the feature space, narrowing it down to the final classification space, facilitating the decision-making process in the final layer.
    
%     \item \textbf{ReLU Activation:} Another ReLU activation is applied after the second linear transformation to introduce additional non-linearity and enhance the model's ability to capture complex patterns.
% \end{enumerate}


% The size of the hidden layers are chosen to be a function of the readout window size with a factor of 4 reduction with respect to the number of input data samples.
The size of the hidden layer is fixed for all readout windows regardless of window size to keep the latency of the model low.
A batch normalization layer is valuable for such an architecture given the bit width of inputs and the use of fixed-point calculations in quantized neural networks to optimize FPGA resources -- described in more detail below.
Among other benefits of batch normalization, scaling the logits prevents computational overflows.  
We demonstrate the performance of two versions of this NN with different hidden neurons to compare performance with respect to model size and complexity. 
The smaller version described in Fig. ~\ref{fig:modelarch} uses 4 hidden neurons, and the other uses 64 hidden neurons. 
Both NNs use the sigmoid function for the output layer. 

% \textcolor{red}{Move this to results?} \textcolor{blue}{I am comfortable either way.} 
We utilized the Adam optimizer \cite{kingma2014adam} and a binary-entropy loss function for optimization, and processed the network's output with a sigmoid function to produce a probability distribution over the classes.
We employed gradient descent with a learning rate of \( 10^{-4} \).
Each training iteration was completed in approximately 29 seconds on NVIDIA A100 GPU. 

\subsection{NN Design Space Exploration}

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{fig/window_size_vs_start_location.pdf}
\caption{Readout window analysis.}
\label{fig:dse_window_size_vs_start_location}
\end{figure}

Figure~\ref{fig:dse_window_size_vs_start_location} shows the fidelity of an optimized neural network (with four hidden neurons) using varying readout window sizes and starting locations. 
The smallest window size is 50 clock cycles (CLK) and increments by 50 CLKs up to 700 CLKs, followed by an evaluation on the full readout window. 
This process is repeated for starting locations, beginning at 0 CLK and increasing in 50 CLK increments up to 350.
The results indicate that starting the readout window later generally improves performance, especially with smaller window sizes. 
However, this improvement plateaus at around 100-150 CLKs. Similarly, larger windows lead to better performance, though the benefits diminish beyond approximately 400 CLKs. 
Based on these findings, we focus on a starting location of 100 CLKs, as it provides high fidelity with the smallest effective window size (400 CLKs). 
We repeated this design space exploration for the second NN version (with 64 hidden neurons), as well as for thresholding and matched filtering methods, observing similar trends as shown in Figure~\ref{fig:dse_window_size_vs_start_location}.

\begin{figure}
    \includegraphics[width=.4\textwidth]{fig/dse_fidelity_vs_param_count.pdf}
    \caption{The impact of model and readout window size on fidelity.}
    \label{fig:dse_params_vs_acc}
\end{figure}


Figure~\ref{fig:dse_params_vs_acc} presents the design space exploration of both 2-layer NN variants, comparing their performance based on the number of trainable parameters and test fidelity across different readout window sizes.
All results are based on data starting at 100 CLKs. The exploration includes window sizes starting from 350 CLKs and increasing in 50 CLK increments, up to 650 CLKs.
As seen in Figure~\ref{fig:dse_window_size_vs_start_location}, the most critical features for state discrimination appear after the first 100 ADC clock cycles. 
Therefore, we exclude the first 100 ADC units in our exploration. 
The graph indicates that test accuracy improves with the number of parameters, reaching a peak at a readout window size of 400 CLKs, beyond which additional parameters provide minimal improvement. 
Both NN variants show similar performance within this range, demonstrating that smaller NNs can achieve the same fidelity as larger architectures, making them more efficient.
Interestingly, the smaller NN variant surpasses the fidelity thresholds for thresholding (TH) and matched filtering (MF) at 400 CLKs, whereas the larger NN achieves this at 450 CLKs. 
This suggests that the smaller NN is less prone to overparameterization and overfitting, making it a more efficient choice for state discrimination and FPGA integration.

Figure~\ref{fig:exp_3} illustrates how fidelity varies as we change the starting position of the 400-CLK readout window of the 2-layer NN with 4 hidden neurons, thresholding, and match filtering methods. 
All methods show a similar trend: fidelity initially increases with the readout start window location, peaks around the 100–150 ADC clock cycle mark, and then gradually declines.
This is consistent with the time it takes to populate the readout resonator, seen previously in the average trajectory data in Fig.~\ref{fig:exp_2}.
When the readout window starts too late, the decrease in fidelity can be associated with qubit $T_1$ decay. 
The NN method generally has a slightly higher fidelity than the TH and MF methods across most locations.
Both methods achieve the highest fidelity when the readout window begins around 100 ADC CLKs. 
Moving forward, we will focus on a 400 CLK readout window starting at 100 CLKs.
% Fig~\ref{fig:exp_3} shows the fidelity of the 800x4x1 with ternary weights with minimal impact to performance compared to MF and TH methods.

\begin{figure}
\centering
\includegraphics[width=.85\columnwidth]{fig/fidelity_vs_window_opt.pdf}
\caption{Optimal neural network with 400 CLK readout window starting at 100. \textcolor{red}{@Javi/Giuseppe: Details of the NN values here - are these for the small model? we should also show a larger model that can reach the same performance as the TH/MF.}}
\label{fig:exp_3}
\end{figure}



\subsection{Hardware optimization}

A co-design approach is taken to optimize neural networks for FPGA implementation. 
Typically, all parameters and data are represented using fixed-point precision, as opposed to the standard 32-bit floating-point notation used during the training and evaluation phases. 
For FPGA deployment, all data is quantized to fixed-point, which results in some level of performance degradation compared to floating-point notation. 
To address this, we employ quantization aware training (QAT). 
This approach helps improve the accuracy of the quantized models on FPGAs by simulating quantization during the training process \cite{jianfei1, jianfei2}. 
Neural networks learn to operate within the constraints of lower precision (e.g., 8-bit integers). 
The benefits of QAT are two-fold: it minimizes the accuracy loss due to quantization and significantly reduces model size, making it easier to deploy on devices with limited memory and hardware resources. 
Quantized models can achieve faster inference times due to the reduced computational complexity of arithmetic operations, which are crucial for real-time processing applications. 
All parameters and activations are quantized using uniform symmetric quantization. 
% Data from the ADC units are not normalized \textcolor{red}{(maybe don't need to emphasize this, mention adding normalization in future iterations for robustness against drifts?)} and are fed directly to the network as 14-bit unsigned integers. 
Data from the ADC units are fed directly to the network as 14-bit unsigned integers. 
In future work, normalizing the ADC data should be studied for robustness against drifts. 
We explore different quantization schemes with 4 hidden neurons (800x4x1) and 64 hidden neurons (800x64x1) as reference. 
Table ~\ref{tab:quant} highlights the trade-offs between model precision (bit-width) and performance. 
Both architectures show stable performance using 32-bit floating point (32FP), with minor variations across CLKs. 
6-bit and 3-bit quantization shows a slight drop compared to 32FP, but remains close. 
Ternary quantization exhibits the lowest values, restricted to -1, 0, or 1. 
It often sacrifices accuracy to reduce model size and complexity, but remains stable given the linearity of single qubit classification. 
We opt to proceed with the 800x4x1 NN using ternary weights to minimize both hardware footprint and latency. 

\begin{table*}[h!]
\centering
\begin{tabular}{|p{2cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|}
\hline
\textbf{Start Location (CLK)} &  \textbf{0} & \textbf{50} & \textbf{100} & \textbf{150} & \textbf{200} & \textbf{250} & \textbf{300} & \textbf{350} \\ \hline
800x64x1 (32FP)     &  0.9141 & 0.9193 & 0.9207 & 0.9186 & 0.9147 & 0.9097 & 0.9035 & 0.8978 \\ \hline
800x4x1 (32FP)    &  0.9143 & 0.9195 & 0.9206 & 0.9187 & 0.9150 & 0.9099 & 0.9034 & 0.8979 \\ \hline
800x4x1 (6b)      &  0.9135 & 0.9193 & 0.9208 & 0.9186 & 0.9146 & 0.9095 & 0.9035 & 0.8975 \\ \hline
800x4x1 (3b)      &  0.9146 & 0.9195 & 0.9207 & 0.9186 & 0.9147 & 0.9097 & 0.9034 & 0.8980 \\ \hline
800x4x1 (teranry) &  0.9134 & 0.9187 & 0.9202 & 0.9180 & 0.9139 & 0.9093 & 0.9032 & 0.8970 \\ \hline
\end{tabular}
\caption{Quantization exploration with 2-layer NN}
\label{tab:quant}
\end{table*}
